High mass function ellipsoidal variables in the Gaia Focused Product Release: searching for black hole candidates in the binary zoo

The recent Gaia Focused Product Release contains radial velocity time-series for more than 9,000 Gaia long-period photometric variables. Here we search for binary systems with large radial velocity amplitudes to identify candidates with massive, unseen companions. Eight targets have binary mass function $f(M)>1\ M_\odot$, three of which are eclipsing binaries. The remaining five show evidence of ellipsoidal modulations. We fit spectroscopic orbit models to the Gaia radial velocities, and fit the spectral energy distributions of three targets. For the two systems most likely to host dark companions, J0946 and J1640, we use PHOEBE to fit the ASAS-SN light curves and Gaia radial velocities. The derived companion masses are $>3 M_\odot$, but the high Galactic dust extinctions towards these objects limit our ability to rule out main sequence companions or subgiants hotter than the photometric primaries. These systems are similar to other stellar-mass black hole impostors, notably the Unicorn (V723 Mon) and the Giraffe (2M04123153$+$6738486). While it is possible that J1640 and J0946 are similar examples of stripped giant star binaries, high-resolution spectra can be used to determine the nature of their companions.

==> ANC/J0946/sed_table_fullJ0946.tex <==
\begin{tabular}{cc r r r r r r r r r r r r r r}
\toprule
{Model} &                    Free &                 Fixed &                Binary &                    Dust \\
\midrule
{$T_{\rm{eff}}$ $(\rm{K})$}    &      $4900^{+70}_{-50}$ &    $4830^{+20}_{-20}$ &    $4180^{+70}_{-90}$ &    $4410^{+120}_{-100}$ \\
{$R$ $(\rm{R}_\odot)$}         &          $31^{+1}_{-1}$ &        $31^{+1}_{-1}$ &  $34.6^{+0.8}_{-0.9}$ &          $28^{+1}_{-1}$ \\
{$L$ $(\rm{L}_\odot)$}         &       $500^{+50}_{-50}$ &     $470^{+40}_{-40}$ &     $330^{+20}_{-30}$ &        $265^{+9}_{-16}$ \\
{$\log g$ }                    &     $2.4^{+0.3}_{-0.3}$ &   $2.4^{+0.3}_{-0.3}$ &     $3.3^{+1}_{-0.7}$ &                      -- \\
{$T_{\rm{eff, 2}}$ $(\rm{K})$} &                      -- &                    -- &  $6700^{+200}_{-400}$ &                      -- \\
{$R_2$ $(\rm{R}_\odot)$}       &                      -- &                    -- &        $10^{+2}_{-1}$ &                      -- \\
{$L_2$ $(\rm{L}_\odot)$}       &                      -- &                    -- &     $180^{+30}_{-20}$ &                      -- \\
{$\log g_2$ }                  &                      -- &                    -- &   $4.1^{+0.6}_{-0.9}$ &                      -- \\
{$A_V$ $(\rm{mag})$}           &  $2.51^{+0.07}_{-0.06}$ &         \textbf{2.41} &         \textbf{2.41} &   $1.39^{+0.05}_{-0.2}$ \\
{Dist $(\rm{pc})$}             &    $4300^{+200}_{-200}$ &  $4300^{+200}_{-200}$ &         \textbf{4297} &                      -- \\
{$\tau_{\nu}$ }                &                      -- &                    -- &                    -- &  $0.22^{+0.05}_{-0.06}$ \\
{$T_{\rm{dust}}$ $(\rm{K})$}   &                      -- &                    -- &                    -- &       $840^{+70}_{-70}$ \\
{$R_{\rm{dust}}$ $(R_\odot)$}  &                      -- &                    -- &                    -- &            $1400\pm300$ \\
{$M_c$ $(M_\odot)$}            &                   0.355 &                 0.352 &                 0.334 &                   0.324 \\
\bottomrule
\end{tabular}


==> ANC/J1640/sed_table_fullJ1640.tex <==
\begin{tabular}{cc r r r r r r r r r r r r r r}
\toprule
{Model} &                    Free &                   Fixed &                  Binary &                    Dust \\
\midrule
{$T_{\rm{eff}}$ $(\rm{K})$}    &      $4080^{+40}_{-40}$ &      $3560^{+20}_{-20}$ &    $3200^{+200}_{-200}$ &      $3910^{+50}_{-50}$ \\
{$R$ $(\rm{R}_\odot)$}         &          $56^{+4}_{-5}$ &          $59^{+5}_{-5}$ &    $60.1^{+0.2}_{-0.2}$ &          $46^{+1}_{-1}$ \\
{$L$ $(\rm{L}_\odot)$}         &     $800^{+100}_{-100}$ &       $500^{+80}_{-80}$ &       $360^{+80}_{-70}$ &       $440^{+20}_{-20}$ \\
{$\log g$ }                    &     $3.0^{+0.1}_{-0.2}$ &  $1.40^{+0.10}_{-0.09}$ &  $0.02^{+0.02}_{-0.01}$ &                      -- \\
{$T_{\rm{eff, 2}}$ $(\rm{K})$} &                      -- &                      -- &      $6710^{+40}_{-80}$ &                      -- \\
{$R_2$ $(\rm{R}_\odot)$}       &                      -- &                      -- &     $4.2^{+0.1}_{-0.1}$ &                      -- \\
{$L_2$ $(\rm{L}_\odot)$}       &                      -- &                      -- &          $32^{+1}_{-1}$ &                      -- \\
{$\log g_2$ }                  &                      -- &                      -- &     $0.4^{+0.5}_{-0.3}$ &                      -- \\
{$A_V$ $(\rm{mag})$}           &  $3.39^{+0.07}_{-0.08}$ &           \textbf{2.25} &           \textbf{2.25} &   $1.77^{+0.2}_{-0.10}$ \\
{Dist $(\rm{pc})$}             &    $3900^{+300}_{-300}$ &    $4000^{+300}_{-300}$ &           \textbf{3809} &                      -- \\
{$\tau_{\nu}$ }                &                      -- &                      -- &                      -- &  $0.68^{+0.09}_{-0.08}$ \\
{$T_{\rm{dust}}$ $(\rm{K})$}   &                      -- &                      -- &                      -- &       $630^{+30}_{-20}$ \\
{$R_{\rm{dust}}$ $(R_\odot)$}  &                      -- &                      -- &                      -- &            $4000\pm500$ \\
{$M_c$ $(M_\odot)$}            &                   0.378 &                   0.354 &                   0.338 &                   0.348 \\
\bottomrule
\end{tabular}

